JSON Web Token (JWT) based client authentication in Message Queuing Telemetry Transport (MQTT)

This paper is an overview of JSON Web Token (JWT) and Transport Layer Security (TLS) as two primary approaches for authentication of the things on the Internet. JSON Web Token (JWT) is used extensively today for authorization and authentication within the OAuth and the OpenId framework. Recently, the Google Cloud IoT has mandated the use of JWT for both HTTP and Message Queuing Telemetry Transport (MQTT) protocol based clients connecting to the cloud service securely over TLS. MQTT is the protocol of choice in IoT devices and is the primary focus of this paper as the application protocol. Another popular cloud platform Amazon Web Service (AWS) uses the TLS mutual authentication for client authentication. Any comparison provided here between the two approaches is primarily from a constrained device client perspective.

==> reference.tex <==
% $ biblatex auxiliary file $
% $ biblatex bbl format version 2.8 $
% Do not modify the above lines!
%
% This is an auxiliary file used by the 'biblatex' package.
% This file may safely be deleted. It will be recreated by
% biber as required.
%
\begin{thebibliography}{1}

\bibitem{Goossens}
Michel Goossens, Frank Mittelbach, and Alexander Samarin.
\newblock {\em The LaTeX Companion}.
\newblock Addison-Wesley, 1 edition, 1994.

\bibitem{adams}
Douglas Adams.
\newblock {\em The Restaurant at the End of the Universe}.
\newblock The Hitchhiker's Guide to the Galaxy. Pan Macmillan, 1980.

\bibitem{feynman}
Richard~P. Feynman.
\newblock Very high-energy collisions of hadrons.
\newblock {\em Phys. Rev. Lett.}, 23:1415--1417, Dec 1969.

\end{thebibliography} % 


\refsection{0}
  \sortlist[entry]{anyt/global/}
    \entry{aws-iam}{report}{}
      \field{labelalpha}{AWS IAM}
      \field{sortinit}{A}
      \field{sortinithash}{3248043b5fe8d0a34dab5ab6b8d4309b}
      \field{labeltitlesource}{title}
      \field{shorthand}{AWS IAM}
      \field{title}{{AWS Identity and Access Management (IAM)}}
      \field{type}{techreport}
      \verb{url}
      \verb https://aws.amazon.com/iam/
      \endverb
    \endentry
    \entry{aws-iot}{report}{}
      \field{labelalpha}{AWS IoT}
      \field{sortinit}{A}
      \field{sortinithash}{3248043b5fe8d0a34dab5ab6b8d4309b}
      \field{labeltitlesource}{title}
      \field{shorthand}{AWS IoT}
      \field{title}{{AWS IoT Developer Guide}}
      \field{type}{techreport}
      \verb{url}
      \verb https://aws.amazon.com/documentation/iot/
      \endverb
    \endentry
    \entry{aws-protocols}{report}{}
      \field{labelalpha}{AWS IoT: Protocol}
      \field{sortinit}{A}
      \field{sortinithash}{3248043b5fe8d0a34dab5ab6b8d4309b}
      \field{labeltitlesource}{title}
      \field{shorthand}{AWS IoT: Protocol}
      \field{title}{{AWS IoT Developer Guide}}
      \field{type}{techreport}
      \verb{url}
      \verb https://docs.aws.amazon.com/iot/latest/developerguide/protocols.html
      \endverb
    \endentry
    \entry{aws-security}{report}{}
      \field{labelalpha}{AWS IoT: Security}
      \field{sortinit}{A}
      \field{sortinithash}{3248043b5fe8d0a34dab5ab6b8d4309b}
      \field{labeltitlesource}{title}
      \field{shorthand}{AWS IoT: Security}
      \field{title}{{AWS IoT Developer Guide: Security \& Identity}}
      \field{type}{techreport}
      \verb{url}
      \verb https://docs.aws.amazon.com/iot/latest/developerguide/iot-security-identity.html
      \endverb
    \endentry
    \entry{kap}{book}{}
      \name{author}{1}{}{%
        {{hash=04136c981effe35c287f453cba3142dd}{%
           family={Colin\bibnamedelima Boyd},
           familyi={C\bibinitperiod\bibinitdelim B\bibinitperiod},
           given={Douglas\bibnamedelima Stebila},
           giveni={D\bibinitperiod\bibinitdelim S\bibinitperiod},
           suffix={Anish\bibnamedelima Mathuria},
           suffixi={A\bibinitperiod\bibinitdelim M\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {Springer}%
      }
      \strng{namehash}{04136c981effe35c287f453cba3142dd}
      \strng{fullhash}{04136c981effe35c287f453cba3142dd}
      \strng{authornamehash}{04136c981effe35c287f453cba3142dd}
      \strng{authorfullhash}{04136c981effe35c287f453cba3142dd}
      \field{labelalpha}{Col18}
      \field{sortinit}{C}
      \field{sortinithash}{095692fd22cc3c74d7fe223d02314dbd}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{title}{Protocols for Authentication and Key Establishment - pre publication draft}
      \field{year}{2018}
    \endentry
    \entry{google-jwt}{report}{}
      \field{labelalpha}{GCS IoT: JWT}
      \field{sortinit}{G}
      \field{sortinithash}{618d986594b7198ba52cf8b00d348f3f}
      \field{labeltitlesource}{title}
      \field{shorthand}{GCS IoT: JWT}
      \field{title}{{Google Cloud: IoT: Using JSON Web Tokens (JWTs)}}
      \field{type}{techreport}
      \verb{url}
      \verb https://cloud.google.com/iot/docs/how-tos/credentials/jwts
      \endverb
    \endentry
    \entry{google-mqtt}{report}{}
      \field{labelalpha}{GCS: IoT}
      \field{sortinit}{G}
      \field{sortinithash}{618d986594b7198ba52cf8b00d348f3f}
      \field{labeltitlesource}{title}
      \field{shorthand}{GCS: IoT}
      \field{title}{{Google Cloud: IoT: Using the MQTT Bridge}}
      \field{type}{techreport}
      \verb{url}
      \verb https://cloud.google.com/iot/docs/how-tos/mqtt-bridge
      \endverb
    \endentry
    \entry{imei-based-authenitcation}{report}{}
      \name{author}{1}{}{%
        {{hash=0d7944530ce384aca2162acbaeb765ca}{%
           family={Jung},
           familyi={J\bibinitperiod},
           given={Seung\bibnamedelimb Wook\bibnamedelimb Jung\bibnamedelimb \&\bibnamedelima Souhwan},
           giveni={S\bibinitperiod\bibinitdelim W\bibinitperiod\bibinitdelim J\bibinitperiod\bibinitdelim \~S\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {International Journal of Distributed Sensor Networks}%
      }
      \strng{namehash}{0d7944530ce384aca2162acbaeb765ca}
      \strng{fullhash}{0d7944530ce384aca2162acbaeb765ca}
      \strng{authornamehash}{0d7944530ce384aca2162acbaeb765ca}
      \strng{authorfullhash}{0d7944530ce384aca2162acbaeb765ca}
      \field{labelalpha}{JWT based Auth}
      \field{sortinit}{J}
      \field{sortinithash}{c86bd6cced82a15683b396c2169909ef}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{shorthand}{JWT based Auth}
      \field{title}{{A Study on a JWT-Based User Authentication and API Assessment Scheme Using IMEI in a Smart Home Environment}}
      \field{type}{techreport}
      \field{year}{2017}
      \verb{url}
      \verb http://www.mdpi.com/2071-1050/9/7/1099
      \endverb
    \endentry
    \entry{mqtt-spec}{report}{}
      \field{labelalpha}{MQTT 3.1.1}
      \field{sortinit}{M}
      \field{sortinithash}{c26a05ef03e4429073ed5c825140fac3}
      \field{labeltitlesource}{title}
      \field{shorthand}{MQTT 3.1.1}
      \field{title}{{MQTT 3.1.1 Specification}}
      \field{type}{techreport}
      \verb{url}
      \verb http://docs.oasis-open.org/mqtt/mqtt/v3.1.1/os/mqtt-v3.1.1-os.html
      \endverb
    \endentry
    \entry{mqtt-sn-spec}{report}{}
      \field{labelalpha}{MQTT-SN 1.2}
      \field{sortinit}{M}
      \field{sortinithash}{c26a05ef03e4429073ed5c825140fac3}
      \field{labeltitlesource}{title}
      \field{shorthand}{MQTT-SN 1.2}
      \field{title}{{MQTT For Sensor Networks (MQTT-SN) Protocol Specification Version 1.2}}
      \field{type}{techreport}
      \verb{url}
      \verb http://mqtt.org/new/wp-content/uploads/2009/06/MQTT-SN_spec_v1.2.pdf
      \endverb
    \endentry
    \entry{personal-oauth}{report}{}
      \name{author}{1}{}{%
        {{hash=ea89fc1c9504bf71ace37e26edd55cb3}{%
           family={Namsu\bibnamedelima Hong},
           familyi={N\bibinitperiod\bibinitdelim H\bibinitperiod},
           given={Moon-Seog\bibnamedelimb Jun\bibnamedelimb \& Jungho\bibnamedelima Kang},
           giveni={M\bibinithyphendelim S\bibinitperiod\bibinitdelim J\bibinitperiod\bibinitdelim \~J\bibinitperiod\bibinitdelim K\bibinitperiod},
           suffix={Mansik\bibnamedelima KimOrcID},
           suffixi={M\bibinitperiod\bibinitdelim K\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {International Journal of Distributed Sensor Networks}%
      }
      \strng{namehash}{ea89fc1c9504bf71ace37e26edd55cb3}
      \strng{fullhash}{ea89fc1c9504bf71ace37e26edd55cb3}
      \strng{authornamehash}{ea89fc1c9504bf71ace37e26edd55cb3}
      \strng{authorfullhash}{ea89fc1c9504bf71ace37e26edd55cb3}
      \field{labelalpha}{OAuth for IoT}
      \field{sortinit}{O}
      \field{sortinithash}{f5d80ef71b5b58852663ecfd775b175a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{shorthand}{OAuth for IoT}
      \field{title}{{Personal OAuth authorization server and push OAuth for Internet of Things}}
      \field{type}{techreport}
      \field{year}{2017}
      \verb{url}
      \verb http://journals.sagepub.com/doi/10.1177/1550147717712627
      \endverb
    \endentry
    \entry{openid-spec}{report}{}
      \field{labelalpha}{OpenID}
      \field{sortinit}{O}
      \field{sortinithash}{f5d80ef71b5b58852663ecfd775b175a}
      \field{labeltitlesource}{title}
      \field{shorthand}{OpenID}
      \field{title}{{OpenID Connect Core 1.0}}
      \field{type}{techreport}
      \verb{url}
      \verb http://openid.net/specs/openid-connect-core-1_0.html
      \endverb
    \endentry
    \entry{rfc-tls-1.0}{report}{}
      \name{author}{1}{}{%
        {{hash=c2785b23ff4dd6670c8ea432278e4f9b}{%
           family={Allen},
           familyi={A\bibinitperiod},
           given={Dierks\bibnamedelima \&},
           giveni={D\bibinitperiod\bibinitdelim \\bibinitperiod}}}%
      }
      \list{institution}{1}{%
        {RFC Editor}%
      }
      \list{publisher}{1}{%
        {RFC Editor}%
      }
      \strng{namehash}{c2785b23ff4dd6670c8ea432278e4f9b}
      \strng{fullhash}{c2785b23ff4dd6670c8ea432278e4f9b}
      \strng{authornamehash}{c2785b23ff4dd6670c8ea432278e4f9b}
      \strng{authorfullhash}{c2785b23ff4dd6670c8ea432278e4f9b}
      \field{labelalpha}{RFC2246}
      \field{sortinit}{R}
      \field{sortinithash}{c15bc8eb6936bc6b3c8baa9e8575af53}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{howpublished}{Internet Requests for Comments}
      \field{month}{01}
      \field{number}{2246}
      \field{shorthand}{RFC2246}
      \field{title}{{The TLS Protocol Version 1.0}}
      \field{type}{{RFC}}
      \field{year}{1999}
      \verb{url}
      \verb http://www.rfc-editor.org/rfc/rfc2246.txt
      \endverb
    \endentry
    \entry{rfc-sntp}{report}{}
      \name{author}{1}{}{%
        {{hash=bf8413517bd150c6f939d01a0f371302}{%
           family={Mills},
           familyi={M\bibinitperiod}}}%
      }
      \list{institution}{1}{%
        {RFC Editor}%
      }
      \list{publisher}{1}{%
        {RFC Editor}%
      }
      \strng{namehash}{bf8413517bd150c6f939d01a0f371302}
      \strng{fullhash}{bf8413517bd150c6f939d01a0f371302}
      \strng{authornamehash}{bf8413517bd150c6f939d01a0f371302}
      \strng{authorfullhash}{bf8413517bd150c6f939d01a0f371302}
      \field{labelalpha}{RFC4330}
      \field{sortinit}{R}
      \field{sortinithash}{c15bc8eb6936bc6b3c8baa9e8575af53}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{howpublished}{Internet Requests for Comments}
      \field{month}{01}
      \field{number}{4330}
      \field{shorthand}{RFC4330}
      \field{title}{{Simple Network Time Protocol (SNTP) Version 4 for IPv4, IPv6 and OSI}}
      \field{type}{{RFC}}
      \field{year}{2006}
      \verb{url}
      \verb http://www.rfc-editor.org/rfc/rfc4330.txt
      \endverb
    \endentry
    \entry{rfc-encoding}{report}{}
      \name{author}{1}{}{%
        {{hash=093dbeb00831d5410279e2d1d6ca5e25}{%
           family={Josefsson},
           familyi={J\bibinitperiod}}}%
      }
      \list{institution}{1}{%
        {RFC Editor}%
      }
      \list{publisher}{1}{%
        {RFC Editor}%
      }
      \strng{namehash}{093dbeb00831d5410279e2d1d6ca5e25}
      \strng{fullhash}{093dbeb00831d5410279e2d1d6ca5e25}
      \strng{authornamehash}{093dbeb00831d5410279e2d1d6ca5e25}
      \strng{authorfullhash}{093dbeb00831d5410279e2d1d6ca5e25}
      \field{labelalpha}{RFC4648}
      \field{sortinit}{R}
      \field{sortinithash}{c15bc8eb6936bc6b3c8baa9e8575af53}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{howpublished}{Internet Requests for Comments}
      \field{month}{10}
      \field{number}{4648}
      \field{shorthand}{RFC4648}
      \field{title}{{The Base16, Base32, and Base64 Data Encodings}}
      \field{type}{{RFC}}
      \field{year}{2006}
      \verb{url}
      \verb http://www.rfc-editor.org/rfc/rfc4648.txt
      \endverb
    \endentry
    \entry{rfc-tls-1.2}{report}{}
      \name{author}{1}{}{%
        {{hash=a927e726d12fa034e44b489464f137d8}{%
           family={Rescorla},
           familyi={R\bibinitperiod},
           given={Dierks\bibnamedelima \&},
           giveni={D\bibinitperiod\bibinitdelim \\bibinitperiod}}}%
      }
      \list{institution}{1}{%
        {RFC Editor}%
      }
      \list{publisher}{1}{%
        {RFC Editor}%
      }
      \strng{namehash}{a927e726d12fa034e44b489464f137d8}
      \strng{fullhash}{a927e726d12fa034e44b489464f137d8}
      \strng{authornamehash}{a927e726d12fa034e44b489464f137d8}
      \strng{authorfullhash}{a927e726d12fa034e44b489464f137d8}
      \field{labelalpha}{RFC5246}
      \field{sortinit}{R}
      \field{sortinithash}{c15bc8eb6936bc6b3c8baa9e8575af53}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{howpublished}{Internet Requests for Comments}
      \field{month}{08}
      \field{number}{5246}
      \field{shorthand}{RFC5246}
      \field{title}{{The Transport Layer Security (TLS) Protocol Version 1.2}}
      \field{type}{{RFC}}
      \field{year}{2008}
      \verb{url}
      \verb http://www.rfc-editor.org/rfc/rfc5246.txt
      \endverb
    \endentry
    \entry{rfc-ntp}{report}{}
      \name{author}{1}{}{%
        {{hash=32e0d349db381a52fc756fbdc89f6a63}{%
           family={al.},
           familyi={a\bibinitperiod},
           given={Mills},
           giveni={M\bibinitperiod},
           prefix={et},
           prefixi={e\bibinitperiod}}}%
      }
      \list{institution}{1}{%
        {RFC Editor}%
      }
      \list{publisher}{1}{%
        {RFC Editor}%
      }
      \strng{namehash}{32e0d349db381a52fc756fbdc89f6a63}
      \strng{fullhash}{32e0d349db381a52fc756fbdc89f6a63}
      \strng{authornamehash}{32e0d349db381a52fc756fbdc89f6a63}
      \strng{authorfullhash}{32e0d349db381a52fc756fbdc89f6a63}
      \field{labelalpha}{RFC5905}
      \field{sortinit}{R}
      \field{sortinithash}{c15bc8eb6936bc6b3c8baa9e8575af53}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{howpublished}{Internet Requests for Comments}
      \field{issn}{2070-1721}
      \field{month}{06}
      \field{number}{5905}
      \field{shorthand}{RFC5905}
      \field{title}{{Network Time Protocol Version 4: Protocol and Algorithms Specification}}
      \field{type}{{RFC}}
      \field{year}{2010}
      \verb{url}
      \verb http://www.rfc-editor.org/rfc/rfc5905.txt
      \endverb
    \endentry
    \entry{rfc-oauth}{report}{}
      \name{author}{1}{}{%
        {{hash=1a637cfc3060504b83462f12f8245420}{%
           family={Hardt},
           familyi={H\bibinitperiod}}}%
      }
      \list{institution}{1}{%
        {RFC Editor}%
      }
      \list{publisher}{1}{%
        {RFC Editor}%
      }
      \strng{namehash}{1a637cfc3060504b83462f12f8245420}
      \strng{fullhash}{1a637cfc3060504b83462f12f8245420}
      \strng{authornamehash}{1a637cfc3060504b83462f12f8245420}
      \strng{authorfullhash}{1a637cfc3060504b83462f12f8245420}
      \field{labelalpha}{RFC6749}
      \field{sortinit}{R}
      \field{sortinithash}{c15bc8eb6936bc6b3c8baa9e8575af53}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{howpublished}{Internet Requests for Comments}
      \field{issn}{2070-1721}
      \field{month}{10}
      \field{number}{6749}
      \field{shorthand}{RFC6749}
      \field{title}{{The OAuth 2.0 Authorization Framework}}
      \field{type}{{RFC}}
      \field{year}{2012}
      \verb{url}
      \verb http://www.rfc-editor.org/rfc/rfc6749.txt
      \endverb
    \endentry
    \entry{rfc-jws}{report}{}
      \name{author}{1}{}{%
        {{hash=a858c3cd054fbd4f30da3d3af03af5f8}{%
           family={al.},
           familyi={a\bibinitperiod},
           given={Jones},
           giveni={J\bibinitperiod},
           prefix={et},
           prefixi={e\bibinitperiod}}}%
      }
      \list{institution}{1}{%
        {RFC Editor}%
      }
      \list{publisher}{1}{%
        {RFC Editor}%
      }
      \strng{namehash}{a858c3cd054fbd4f30da3d3af03af5f8}
      \strng{fullhash}{a858c3cd054fbd4f30da3d3af03af5f8}
      \strng{authornamehash}{a858c3cd054fbd4f30da3d3af03af5f8}
      \strng{authorfullhash}{a858c3cd054fbd4f30da3d3af03af5f8}
      \field{labelalpha}{RFC7515}
      \field{sortinit}{R}
      \field{sortinithash}{c15bc8eb6936bc6b3c8baa9e8575af53}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{howpublished}{Internet Requests for Comments}
      \field{issn}{2070-1721}
      \field{month}{05}
      \field{number}{7519}
      \field{shorthand}{RFC7515}
      \field{title}{{JSON Web Signature (JWS)}}
      \field{type}{{RFC}}
      \field{year}{2015}
      \verb{url}
      \verb http://www.rfc-editor.org/rfc/rfc7515.txt
      \endverb
    \endentry
    \entry{rfc-jwe}{report}{}
      \name{author}{1}{}{%
        {{hash=15849dc08f21b77ea240c172d4a26116}{%
           family={{Jones\bibnamedelimb \& Hildebrand}.},
           familyi={J\bibinitperiod}}}%
      }
      \list{institution}{1}{%
        {RFC Editor}%
      }
      \list{publisher}{1}{%
        {RFC Editor}%
      }
      \strng{namehash}{15849dc08f21b77ea240c172d4a26116}
      \strng{fullhash}{15849dc08f21b77ea240c172d4a26116}
      \strng{authornamehash}{15849dc08f21b77ea240c172d4a26116}
      \strng{authorfullhash}{15849dc08f21b77ea240c172d4a26116}
      \field{labelalpha}{RFC7516}
      \field{sortinit}{R}
      \field{sortinithash}{c15bc8eb6936bc6b3c8baa9e8575af53}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{howpublished}{Internet Requests for Comments}
      \field{issn}{2070-1721}
      \field{month}{05}
      \field{number}{7519}
      \field{shorthand}{RFC7516}
      \field{title}{{JSON Web Encryption (JWE)}}
      \field{type}{{RFC}}
      \field{year}{2015}
      \verb{url}
      \verb http://www.rfc-editor.org/rfc/rfc7516.txt
      \endverb
    \endentry
    \entry{rfc-alg}{report}{}
      \name{author}{1}{}{%
        {{hash=59830e37ce261d31ad0da0d5d270d0e1}{%
           family={Jones},
           familyi={J\bibinitperiod}}}%
      }
      \list{institution}{1}{%
        {RFC Editor}%
      }
      \list{publisher}{1}{%
        {RFC Editor}%
      }
      \strng{namehash}{59830e37ce261d31ad0da0d5d270d0e1}
      \strng{fullhash}{59830e37ce261d31ad0da0d5d270d0e1}
      \strng{authornamehash}{59830e37ce261d31ad0da0d5d270d0e1}
      \strng{authorfullhash}{59830e37ce261d31ad0da0d5d270d0e1}
      \field{labelalpha}{RFC7518}
      \field{sortinit}{R}
      \field{sortinithash}{c15bc8eb6936bc6b3c8baa9e8575af53}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{howpublished}{Internet Requests for Comments}
      \field{issn}{2070-1721}
      \field{month}{05}
      \field{number}{7518}
      \field{shorthand}{RFC7518}
      \field{title}{{JSON Web Algorithms}}
      \field{type}{{RFC}}
      \field{year}{2015}
      \verb{url}
      \verb http://www.rfc-editor.org/rfc/rfc7518.txt
      \endverb
    \endentry
    \entry{rfc-jwt}{report}{}
      \name{author}{1}{}{%
        {{hash=a858c3cd054fbd4f30da3d3af03af5f8}{%
           family={al.},
           familyi={a\bibinitperiod},
           given={Jones},
           giveni={J\bibinitperiod},
           prefix={et},
           prefixi={e\bibinitperiod}}}%
      }
      \list{institution}{1}{%
        {RFC Editor}%
      }
      \list{publisher}{1}{%
        {RFC Editor}%
      }
      \strng{namehash}{a858c3cd054fbd4f30da3d3af03af5f8}
      \strng{fullhash}{a858c3cd054fbd4f30da3d3af03af5f8}
      \strng{authornamehash}{a858c3cd054fbd4f30da3d3af03af5f8}
      \strng{authorfullhash}{a858c3cd054fbd4f30da3d3af03af5f8}
      \field{labelalpha}{RFC7519}
      \field{sortinit}{R}
      \field{sortinithash}{c15bc8eb6936bc6b3c8baa9e8575af53}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{howpublished}{Internet Requests for Comments}
      \field{issn}{2070-1721}
      \field{month}{05}
      \field{number}{7519}
      \field{shorthand}{RFC7519}
      \field{title}{{JSON Web Token (JWT)}}
      \field{type}{{RFC}}
      \field{year}{2015}
      \verb{url}
      \verb http://www.rfc-editor.org/rfc/rfc7519.txt
      \endverb
    \endentry
    \entry{rfc-client-authentication}{report}{}
      \name{author}{1}{}{%
        {{hash=2c6da8249c463f3a78780d18725a85f0}{%
           family={al.},
           familyi={a\bibinitperiod},
           given={Campbell},
           giveni={C\bibinitperiod},
           prefix={et},
           prefixi={e\bibinitperiod}}}%
      }
      \list{institution}{1}{%
        {RFC Editor}%
      }
      \list{publisher}{1}{%
        {RFC Editor}%
      }
      \strng{namehash}{2c6da8249c463f3a78780d18725a85f0}
      \strng{fullhash}{2c6da8249c463f3a78780d18725a85f0}
      \strng{authornamehash}{2c6da8249c463f3a78780d18725a85f0}
      \strng{authorfullhash}{2c6da8249c463f3a78780d18725a85f0}
      \field{labelalpha}{RFC7521}
      \field{sortinit}{R}
      \field{sortinithash}{c15bc8eb6936bc6b3c8baa9e8575af53}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{howpublished}{Internet Requests for Comments}
      \field{issn}{2070-1721}
      \field{month}{05}
      \field{number}{7521}
      \field{shorthand}{RFC7521}
      \field{title}{{Assertion Framework for OAuth 2.0 Client Authentication and Authorization Grants}}
      \field{type}{{RFC}}
      \field{year}{2015}
      \verb{url}
      \verb http://www.rfc-editor.org/rfc/rfc7521.txt
      \endverb
    \endentry
    \entry{rfc-json}{report}{}
      \name{author}{1}{}{%
        {{hash=374946fb3a9b52a41dc2fbe302fc8e4c}{%
           family={Bray},
           familyi={B\bibinitperiod}}}%
      }
      \list{institution}{1}{%
        {RFC Editor}%
      }
      \list{publisher}{1}{%
        {RFC Editor}%
      }
      \strng{namehash}{374946fb3a9b52a41dc2fbe302fc8e4c}
      \strng{fullhash}{374946fb3a9b52a41dc2fbe302fc8e4c}
      \strng{authornamehash}{374946fb3a9b52a41dc2fbe302fc8e4c}
      \strng{authorfullhash}{374946fb3a9b52a41dc2fbe302fc8e4c}
      \field{labelalpha}{RFC8259}
      \field{sortinit}{R}
      \field{sortinithash}{c15bc8eb6936bc6b3c8baa9e8575af53}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{howpublished}{Internet Requests for Comments}
      \field{issn}{2070-1721}
      \field{month}{05}
      \field{number}{8259}
      \field{shorthand}{RFC8259}
      \field{title}{{The JavaScript Object Notation (JSON) Data Interchange Format}}
      \field{type}{{RFC}}
      \field{year}{2015}
      \verb{url}
      \verb http://www.rfc-editor.org/rfc/rfc8259.txt
      \endverb
    \endentry
    \entry{tamarin-prover}{report}{}
      \list{publisher}{1}{%
        {GitHub Reposiroty}%
      }
      \field{labelalpha}{Tamarin prover}
      \field{sortinit}{T}
      \field{sortinithash}{2e5c2f51f7fa2d957f3206819bf86dc3}
      \field{labeltitlesource}{title}
      \field{shorthand}{Tamarin prover}
      \field{title}{{Tamarin prover}}
      \field{type}{techreport}
      \verb{url}
      \verb https://tamarin-prover.github.io/
      \endverb
    \endentry
  \endsortlist
\endrefsection
\endinput

